Putting the Semantics into Semantic Versioning

The long-standing aspiration for software reuse has made astonishing strides in the past few years. Many modern software development ecosystems now come with rich sets of publicly-available components contributed by the community. Downstream developers can leverage these upstream components, boosting their productivity. However, components evolve at their own pace. This imposes obligations on and yields benefits for downstream developers, especially since changes can be breaking, requiring additional downstream work to adapt to. Upgrading too late leaves downstream vulnerable to security issues and missing out on useful improvements; upgrading too early results in excess work. Semantic versioning has been proposed as an elegant mechanism to communicate levels of compatibility, enabling downstream developers to automate dependency upgrades. While it is questionable whether a version number can adequately characterize version compatibility in general, we argue that developers would greatly benefit from tools such as semantic version calculators to help them upgrade safely. The time is now for the research community to develop such tools: large component ecosystems exist and are accessible, component interactions have become observable through automated builds, and recent advances in program analysis make the development of relevant tools feasible. In particular, contracts (both traditional and lightweight) are a promising input to semantic versioning calculators, which can suggest whether an upgrade is likely to be safe.

==> about-version-numbers.tex <==
\section{Towards Semantic Semantic Versioning}
\label{sec:version-numbers}


%\todo[inline]{PL: I've been referring to generalized tools throughout. I think code contracts fall under the definition of ``generalized tool'' that I've been using. I'll make that explicit in the intro; added: ``We use a generalized meaning of ``tool'' which includes not just a concrete program that one executes on one's software but abstract methods and concepts as well.''}

% this exists in the cross-reffed sections so it can go away here.
%Code contracts, discussed in Section~\ref{sec:about-contracts}, are a popular tool for summarizing program behaviour and, we claim, can be used to express version compatibility. Even in the common situation where $A$ and $A'$ don't come with formalized contracts, their clients certainly expect them to adhere to some kind of contracts, or at least informal expectations. As discussed in Section~\ref{sec:api-surfaces}, the scope of relevant changes depends on which open-world versus closed-world assumptions one takes.

% This is in the new section 6.
%Upstream's responsibility is to all clients (or perhaps to reasonable clients). Downstream, at a specific client $C$, only changes from upstream that affect $C$ matter (the approach taken by~\cite{DBLP:conf/sigsoft/McCamantE03}). However, $C$ is affected by all of the upstream components that it uses.
%At the very least, all components export some sort of API to their clients, and Section~\ref{sec:api-surfaces} discussed how much of the API is relevant for upgrades. 
%In any case, new version $A'$ may change the relevant contracts of $A$ by widening them, loosening them, or making incomparable changes to them. Version $A'$ may also change its conformance to any explicitly specified contract that $A$ previously complied to. Section~\ref{sec:taxonomy} proposed important aspects to be included in taxonomies of breaking changes.



\tikzstyle{block} = [rectangle, draw, 
    text width=5em, text centered, rounded corners, minimum height=2em]
\tikzstyle{bt} = [rectangle, draw, 
    text width=1em, text centered, rounded corners, minimum height=2em]
\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta}

\begin{figure*}[h]
  \begin{tikzpicture}
    \node[bt] (A) {$A$};
    \node[bt,below of=A] (A') {$A'$};
    \node[block, right of=A, text width=3em, xshift=1.5em] (Tool1) { Tool 1 };
    \node[block, right of=A', text width=3em, xshift=1.5em] (Tool2) { Tool 2 };
    \node[block, right of=Tool1, text width=5em, xshift=3em] (F1) { Structural Facts };
    \node[block, right of=Tool2, text width=5em, xshift=3em] (F2) { Behavioural Facts };
    \node[block, above right of=F2, text width=5em, xshift=5em] (R) {Reasoning};
    \node[block, right of=R, text width=5em, xshift=4em] (I) {Impacts $A \rightarrow A'$ {\bf Breaking}};

    \draw[->] (A) -- (A') {};
    \draw[-Latex] let
      \p1 = ($ (A') - (A) $),
      \n2 = {veclen(\x1, \y1)*.5}
    in
      (A)++(0,-\n2) -- (Tool1);
    \draw[-Latex] let
      \p1 = ($ (A') - (A) $),
      \n2 = {veclen(\x1, \y1)*.5}
    in
      [-Latex] (A)++(0,-\n2) -- (Tool2);
    \draw[-Latex]  (Tool1) -- (F1);
    \draw[-Latex]  (Tool2) -- (F2);
    \draw[-Latex]  (F1) -- (R);
    \draw[-Latex]  (F2) -- (R);
    \draw[-Latex]  (R) -- (I);
  \end{tikzpicture}
  \caption{Parts of a semantic version calculator. Analysis tools analyze the differences between versions $A$ and $A'$ of a component, producing
    facts which can be manipulated by reasoning tools. Developers can read off the impacts of their changes,
    including whether the change is breaking or not.}
  \label{fig:calculator}
\end{figure*}


\paragraph{Computing version numbers.}
There are many ways to map concrete program changes onto members of a taxonomy like the one we proposed in the previous section. Here is one approach, depicted in Figure~\ref{fig:calculator}. Tools (like the static analysis tools discussed in Section~\ref{sec:about-contracts}) would extract a summary the relevant changes that have occurred in 
an upgraded component. 

For instance, such a summary could consist of Datalog facts instantiating predicates corresponding to the elements of the taxonomy.   Datalog rules could then be applied to compute compatibility levels, and the kind of version change required. The advantage of such an approach is that communities can define policies that suit them, based on developer culture, community practices, and the availability of tools. Using a representation like Datalog has the advantage that those rules can be expressed in an easy-to-understand fashion, while they still have a precisely defined meaning based on Datalog's fixpoint semantics. Other representations, such as more powerful formal ontology languages based on description logics, are possible as well.

% These facts would then be reinterpreted as appropriate predicates. These predicates would be suitable for use by Datalog (or more powerful formal ontology languages based on description logics). The Datalog taxonomy would know about breaking change categories and relationships between predicates, and this knowledge would be expressed in an easy-to-understand fashion.

% \todo[inline]{from elsewhere, could go here: the idea of complementing a verifying compiler with a verifying linker that diffs specs}

Such an approach can only work if the facts can be practically extracted and if they accurately reflect the status of the software. For most languages, facts in the \textit{structural} and \textit{auxiliary} categories can be extracted using a lightweight static analysis of the program (structural) and of its metadata (auxiliary---package manifests, build scripts, etc.).  Changed resourcing requirements can be captured by means of dynamic analysis such as tests, if reasonable levels of test coverage and realistic program inputs are available. The most difficult category is \textit{behavioural}. Tools to analyze behavioural changes must work at a deeper, semantic level, integrating explicit and inferred contracts, which are verified with sophisticated static and dynamic analyses. Program analyses to detect such changes have to make compromises between precision, recall and speed. As discussed earlier, composite or hybrid analyses promise to extract useful facts in this category.

We believe that there ought to exist tool support for evaluating version compatibility at all levels. Today's tools, such as \textit{clirr}, \textit{Revapi}, \textit{rust-semverver}, and \textit{elm bump}, work at a relatively shallow level. 

% Jens: I commented this out, that looked more like a note
%(npm's semantic-release package takes another approach, similar to the .NET platform, and requires developers to annotate commits as being fixes, features, breaking changes, etc.)

% \todo[inline]{Note: That last paragraph leads well into the conclusion.}

%% \todo[inline]{djp:  We need some attempt to argue against the semantic versioning
%%   manifesto, and motivate that something more pragmatic is
%%   needed.}

%% \todo[inline]{djp: Perhaps giving some examples to illustrate what we mean.
%%   Could reference the similarity with the approach to coding styles
%%   taken in the Power of Ten. \url{https://en.wikipedia.org/wiki/The_Power_of_10:_Rules_for_Developing_Safety-Critical_Code} PL: Hmm, I don't think we can credibly argue to limit programmers' expressive power.}


%% \todo[inline]{We also talked about these: maven;
%%   NuGet; and Packagist. The last two are compatible with semver but I don't think they have calculators of any sort. I'll throw in the MSR text in a comment below. I think I'm fine with what we have said so far about similar tools.}


%% • (Maven).  Revapi 13 , Clirr 14 , the Java API Compliance Checker
%% (JAPICC) 15 and the semantic-versioning 16 library are all tools, like
%% rust-semverver, for checking backwards compatibility.  17

%% • (NPM) The tool semantic-release provides the main example here, and
%% all others found either extend this or are plugins for it. This tool
%% determines the next suitable version using commit messages to deter-
%% mine the extent of changes. For example, if one puts “BREAKING CHANGE”
%% in a commit message, then it increments the major version, etc.

%% • (NuGet) The three tools found here, SemVer.FromAssembly 18 ,
%% SemVerAdvisor 19 and SpiseMisu.SemanticVersioning 20 all check
%% backwards compatibility based on exposed API surface.

%% • (Packagist) Here the only tool identified was semcrement which
%% “compares structure definitions of your project’s code in between
%% commits” 21 .

%% 15 https://github.com/lvc/japi-compliance-checker
%% 16 https://github.com/jeluard/semantic-versioning
%% 17 https://www.npmjs.com/package/semantic-release
%% 18 https://www.nuget.org/packages/SemVer.FromAssembly/
%% 19 https://www.nuget.org/packages/SemVerAdvisor/
%% 20 https://www.nuget.org/packages/SpiseMisu.SemanticVersioning/
%% 21 https://packagist.org/packages/wick-ed/semcrement


%% We propose the following way of thinking about contracts in our context:
%% \begin{itemize}
%% \item {\bf What}: types of contracts;
%% \item {\bf How}: types of analysis to detect contracts and conformance with them;
%% \item {\bf Where}: the API surface to which the contracts apply (or where relevant contracts live).
%% \end{itemize}

%% As part of ``what'' we can also think of the level of specification (formal contracts, no contracts, inferred contracts, under-specified contracts, over-specified contracts).


==> contract-deltas.tex <==
\section{Detecting Changes}

In the previous section, we discussed what contracts exist, how to detect them, and where they apply. We now revisit contract detection in the context of inter-version changes to contract definitions and implementations and the implications on version compatibility. 

\todo[inline] {I think the following should now go into Section 3. Or maybe we should split section 3 into a short section about contracts and versioning, and then a section/subsections about what/how/where, and then in this section we discuss changes.}

\todo[inline] {Jens: Detecting and Classifying ? }



==> design.tex <==
\section{Design for Change}



\todo[inline] {Jens: could go into Challenges}

==> dirtree.tex <==
%%
%% This is file `dirtree.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% dirtree.dtx  (with options: `tex')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from dirtree.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file dirtree.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Package `dirtree.dtx'
%% -----------------------------------------------
%% Copyright (C) 2004-2009 Jean-C\^ome Charpentier
%% -----------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% See CTAN archives in directory macros/latex/base/lppl.txt.
%%
%% CONTENTS:
%%   This work consists of the files dirtree.ins and dirtree.dtx.
%%   Derived files are dirtree.tex and dirtree.sty.
%%
%% DESCRIPTION:
%%   dirtree is a package displaying directory trees.
%%
 \def\fileversion{0.32}
 \def\filedate{2012/12/11}
\message{`dirtree' v\fileversion, \filedate\space (jcc)}
\edef\DTAtCode{\the\catcode`\@}
\catcode`\@=11
\long\def\DT@loop#1\DT@repeat{%
  \def\DT@iterate{#1\relax\expandafter\DT@iterate\fi}%
  \DT@iterate
  \let\DT@iterate\relax
}
\let\DT@repeat=\fi
\expandafter\ifx\csname DT@fromsty\endcsname\relax
  \def\@namedef#1{\expandafter\def\csname #1\endcsname}
  \def\@nameuse#1{\csname #1\endcsname}
  \long\def\@gobble#1{}
\fi
\def\@nameedef#1{\expandafter\edef\csname #1\endcsname}
\newdimen\DT@offset \DT@offset=0.2em
\newdimen\DT@width \DT@width=1em
\newdimen\DT@sep \DT@sep=0.2em
\newdimen\DT@all
\DT@all=\DT@offset
\advance\DT@all \DT@width
\advance\DT@all \DT@sep
\newdimen\DT@rulewidth \DT@rulewidth=0.4pt
\newdimen\DT@dotwidth \DT@dotwidth=1.6pt
\newdimen\DTbaselineskip \DTbaselineskip=\baselineskip
\newcount\DT@counti
\newcount\DT@countii
\newcount\DT@countiii
\newcount\DT@countiv
\def\DTsetlength#1#2#3#4#5{%
  \DT@offset=#1\relax
  \DT@width=#2\relax
  \DT@sep=#3\relax
  \DT@all=\DT@offset
  \advance\DT@all by\DT@width
  \advance\DT@all by\DT@sep
  \DT@rulewidth=#4\relax
  \DT@dotwidth=#5\relax
}
\expandafter\ifx\csname DT@fromsty\endcsname\relax
  \def\DTstyle{\tt}
  \def\DTstylecomment{\rm}
\else
  \def\DTstyle{\ttfamily}
  \def\DTstylecomment{\rmfamily}
\fi
\def\DTcomment#1{%
  \kern\parindent\dotfill
  {\DTstylecomment{#1}}%
}
\newdimen\DT@indent
\newdimen\DT@parskip
\newdimen\DT@baselineskip
\def\dirtree#1{%
  \DT@indent=\parindent
  \parindent=\z@
  \DT@parskip=\parskip
  \parskip=\z@
  \DT@baselineskip=\baselineskip
  \baselineskip=\DTbaselineskip
  \let\DT@strut=\strut
  \def\strut{\vrule width\z@ height0.7\baselineskip depth0.3\baselineskip}%
  \DT@counti=\z@
  \let\next\DT@readarg
  \next#1\@nil
  \dimen\z@=\hsize
  \advance\dimen\z@ -\DT@offset
  \advance\dimen\z@ -\DT@width
  \setbox\z@=\hbox to\dimen\z@{%
    \hsize=\dimen\z@
    \vbox{\@nameuse{DT@body@1}}%
  }%
  \dimen\z@=\ht\z@
  \advance\dimen0 by\dp\z@
  \advance\dimen0 by-0.7\baselineskip
  \ht\z@=0.7\baselineskip
  \dp\z@=\dimen\z@
  \par\leavevmode
  \kern\DT@offset
  \kern\DT@width
  \box\z@
  \endgraf
  \DT@countii=\@ne
  \DT@countiii=\z@
  \dimen3=\dimen\z@
  \@namedef{DT@lastlevel@1}{-0.7\baselineskip}%
  \loop
  \ifnum\DT@countii<\DT@counti
    \advance\DT@countii \@ne
    \advance\DT@countiii \@ne
    \dimen\z@=\@nameuse{DT@level@\the\DT@countii}\DT@all
    \advance\dimen\z@ by\DT@offset
    \advance\dimen\z@ by-\DT@all
    \leavevmode
    \kern\dimen\z@
    \DT@countiv=\DT@countii
    \count@=\z@
    \DT@loop
      \advance\DT@countiv \m@ne
      \ifnum\@nameuse{DT@level@\the\DT@countiv} >
        \@nameuse{DT@level@\the\DT@countii}\relax
      \else
        \count@=\@ne
      \fi
    \ifnum\count@=\z@
    \DT@repeat
    \edef\DT@hsize{\the\hsize}%
    \count@=\@nameuse{DT@level@\the\DT@countii}\relax
    \dimen\z@=\count@\DT@all
    \advance\hsize by-\dimen\z@
    \setbox\z@=\vbox{\@nameuse{DT@body@\the\DT@countii}}%
    \hsize=\DT@hsize
    \dimen\z@=\ht\z@
    \advance\dimen\z@ by\dp\z@
    \advance\dimen\z@ by-0.7\baselineskip
    \ht\z@=0.7\baselineskip
    \dp\z@=\dimen\z@
    \@nameedef{DT@lastlevel@\the\DT@countii}{\the\dimen3}%
    \advance\dimen3 by\dimen\z@
    \advance\dimen3 by0.7\baselineskip
    \dimen\z@=\@nameuse{DT@lastlevel@\the\DT@countii}\relax
    \advance\dimen\z@ by-\@nameuse{DT@lastlevel@\the\DT@countiv}\relax
    \advance\dimen\z@ by0.3\baselineskip
    \ifnum\@nameuse{DT@level@\the\DT@countiv} <
        \@nameuse{DT@level@\the\DT@countii}\relax
      \advance\dimen\z@ by-0.5\baselineskip
    \fi
    \kern-0.5\DT@rulewidth
    \hbox{\vbox to\z@{\vss\hrule width\DT@rulewidth height\dimen\z@}}%
    \kern-0.5\DT@rulewidth
    \kern-0.5\DT@dotwidth
    \vrule width\DT@dotwidth height0.5\DT@dotwidth depth0.5\DT@dotwidth
    \kern-0.5\DT@dotwidth
    \vrule width\DT@width height0.5\DT@rulewidth depth0.5\DT@rulewidth
    \kern\DT@sep
    \box\z@
    \endgraf
  \repeat
  \parindent=\DT@indent
  \parskip=\DT@parskip
  \baselineskip=\DT@baselineskip
  \let\strut\DT@strut
}
\def\DT@readarg.#1 #2. #3\@nil{%
  \advance\DT@counti \@ne
  \@namedef{DT@level@\the\DT@counti}{#1}%
  \@namedef{DT@body@\the\DT@counti}{\strut{\DTstyle{#2}\strut}}%
  \ifx\relax#3\relax
    \let\next\@gobble
  \fi
  \next#3\@nil
}
\catcode`\@=\DTAtCode\relax
\endinput
%%
%% End of file `dirtree.tex'.

